IDEAL: Inexact DEcentralized Accelerated Augmented Lagrangian Method

We introduce a framework for designing primal methods under the decentralized optimization setting where local functions are smooth and strongly convex. Our approach consists of approximately solving a sequence of sub-problems induced by the accelerated augmented Lagrangian method, thereby providing a systematic way for deriving several well-known decentralized algorithms including EXTRA arXiv:1404.6264 and SSDA arXiv:1702.08704. When coupled with accelerated gradient descent, our framework yields a novel primal algorithm whose convergence rate is optimal and matched by recently derived lower bounds. We provide experimental results that demonstrate the effectiveness of the proposed algorithm on highly ill-conditioned problems.

==> [Neurips20] Decentralized Acc-AL algorithm /notations.tex <==
\newcommand{\defeq}{\mathrel{\mathop:}=}
\newcommand{\note}[1]{\textcolor{red}{#1}}


\newcommand{\ingd}{\textsc{Ingd}\xspace}
% Operator

\newcommand{\vect}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\mat}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\grad}{\nabla}
\newcommand{\hess}{\nabla^2}
% \newcommand{\argmin}{\mathop{\rm argmin}}
% \newcommand{\argmax}{\mathop{\rm argmax}}
\newcommand{\fracpar}[2]{\frac{\partial #1}{\partial  #2}}
\newcommand{\iprod}[2]{\langle #1, #2 \rangle}

\newcommand{\abs}[1]{\left|{#1}\right|}
% \newcommand{\norm}[1]{\left\|{#1}\right\|}
% \newcommand{\fnorm}[1]{\left\|{#1}\right\|_{\text{F}}}
% \newcommand{\spnorm}[2]{\left\| {#1} \right\|_{\text{S}({#2})}}
\newcommand{\norm}[1]{\|{#1} \|}
\newcommand{\fnorm}[1]{\|{#1} \|_{\text{F}}}
\newcommand{\spnorm}[2]{\| {#1} \|_{\text{S}({#2})}}
\newcommand{\sigmin}{\sigma_{\min}}
\newcommand{\tr}{\mathrm{tr}}
\renewcommand{\det}{\mathrm{det}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\logdet}{\mathrm{logdet}}
\newcommand{\trans}{^{\top}}
\newcommand{\poly}{\mathrm{poly}}
\newcommand{\polylog}{\mathrm{polylog}}
\newcommand{\st}{\mathrm{s.t.~}}
\newcommand{\proj}{\mathcal{P}}
\newcommand{\projII}{\mathcal{P}_{\parallel}}
\newcommand{\projT}{\mathcal{P}_{\perp}}
\newcommand{\floor}[1]{\lfloor {#1} \rfloor}

% Big O
\newcommand{\cO}{\mathcal{O}}
\newcommand{\tlO}{\mathcal{\tilde{O}}}
\newcommand{\tlOmega}{\tilde{\Omega}}
\newcommand{\tlTheta}{\tilde{\Theta}}


% Set

\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Sn}{\mathbb{S}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\E}{\mathbb{E}}
\renewcommand{\Pr}{\mathbb{P}}
\newcommand{\Var}{\text{Var}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\G}{\mathcal{G}}
\newcommand{\Y}{\mathcal{Y}}


% Matrix and Vector

\newcommand{\A}{\mat{A}}
\newcommand{\B}{\mat{B}}
\newcommand{\Q}{\mat{Q}}


\newcommand{\I}{\mat{I}}
\newcommand{\D}{\mat{D}}
\newcommand{\U}{\mat{U}}
\newcommand{\V}{\mat{V}}
\newcommand{\W}{\mat{W}}
\newcommand{\X}{\mat{X}}
\newcommand{\bfGamma}{\mat{\Gamma}}
\newcommand{\bfLambda}{\mat{\Lambda}}
\newcommand{\bfOmega}{\mat{\Omega}}
\newcommand{\e}{\vect{e}}
\renewcommand{\u}{\vect{u}}
\renewcommand{\v}{\vect{v}}
\newcommand{\w}{\vect{w}}
\newcommand{\x}{\vect{x}}
\newcommand{\y}{\vect{y}}
\newcommand{\z}{\vect{z}}
\newcommand{\g}{\vect{g}}
\newcommand{\zero}{\vect{0}}
\newcommand{\fI}{\mathfrak{I}}
\newcommand{\fS}{\mathfrak{S}}
\newcommand{\fE}{\mathfrak{E}}
\newcommand{\fF}{\mathfrak{F}}


% Special Character

\newcommand{\M}{\mathcal{M}}
\renewcommand{\L}{\mathcal{L}}
\renewcommand{\H}{\mathcal{H}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cS}{\mathcal{S}}

\newcommand{\cn}{\kappa}
\newcommand{\nn}{\nonumber}


% Arg<x>
\DeclareMathOperator*{\argmin}{arg\,min} % * Places subscript directly 
%under operator
\DeclareMathOperator*{\argmax}{arg\,max}             
\DeclareMathOperator*{\arginf}{arg\,inf} 
\DeclareMathOperator*{\argsup}{arg\,sup} 

\newlength\myindent
\setlength\myindent{2em}
\newcommand\bindent{%
  \begingroup
  \setlength{\itemindent}{\myindent}
  \addtolength{\algorithmicindent}{\myindent}
}
\newcommand\eindent{\endgroup}
\newcommand{\our}{IDEAL}
\newcommand{\mixing}{mixing }


\newcommand{\eh}{{\color{red}[eqref here]}}

%:) harika tesekkurler.
\definecolor{darkblue}{rgb}{0,0,0.6}
\def\yacomment#1{\textcolor{darkblue}{[ya: #1]}}

% added by Mert for editing
\def\mg#1{\textcolor{purple}{#1}}
% \usepackage[normalem]{ulem}
%\newcommand{\mtodo}[1]{\todo[inline]{ \textbf{MG: } #1 }}
% \usepackage{todonotes}
%%%%% Hongzhou: the todo package introduces some undesirable phenomenon on overleaf, so I remove it %%%%%%
\newcommand{\mtodo}[1]{{\color{red} [MG: #1] }}
\newcommand{\citn}{{\color{red}[Citation]}}

\newcommand{\joan}[1]{{\color{cyan}[JB: #1]}}
\def\bccomment#1{\textcolor{orange}{[bc:#1]}}
\newcommand{\hz}[1]{{\color{magenta}[HZ: #1]}}

==> [Neurips20] Decentralized Acc-AL algorithm /sections/sec1_intro.tex <==
\section{Introduction}
Due to their rapidly increasing size, modern datasets are typically collected, stored and manipulated in a distributed manner. This, together with strict privacy requirements, has created a large demand for efficient solvers for the decentralized setting in which models are trained locally at each agent, and only local parameter vectors are shared. This approach has become particularly appealing for applications such as edge computing~\cite{shi2016edge,mao2017survey}, cooperative multi-agent learning~\cite{bernstein2002complexity, panait2005cooperative} and federated learning~\cite{mcmahan2017communication,shokri2015privacy}.
% , where  strict communication and privacy constraints are imposed. 
Clearly, the nature of the decentralized setting prevents a global synchronization, as only communication within the neighboring machines is allowed. The goal is  then to  arrive at a consensus on all local agents with a model that performs as well as in the centralized setting. 

% The rapid growth of modern datasets, collected in a distributed manner through multiple agents such as smart phones, wearable sensors or drones, %as well as privacy requirements %\mg{over collected data with different sensing devices (such as smart phones, tablets or sensors)},
% have created an increasing demand for efficient learning algorithms. When the data is widely distributed or privacy sensitive, centralized computation is either impractical or prohibited. At this point, decentralized machine learning comes to the rescue: the models are trained locally at each agent, and only the parameter vectors of the local objective functions are shared. This approach has become particularly appealing for applications such as edge computing~\cite{shi2016edge,mao2017survey}, cooperative multi-agent learning~\cite{bernstein2002complexity, panait2005cooperative} and federated learning~\cite{mcmahan2017communication,shokri2015privacy}.
% % , where  strict communication and privacy constraints are imposed. 
% Clearly, the nature of decentralized settings prevents a global synchronization, and only communication within the neighboring agents is allowed. The goal is  then to  arrive at a consensus on all the local agents efficiently with a model that performs as well as in the centralized setting. 



Arguably, the simplest approach for addressing decentralized settings is to adapt the vanilla gradient descent method to the underlying network architecture  \cite{xiao2007distributed, nedic2009distributed, duchi2011dual, jakovetic2014fast}. To this end, the connections between the agents are modeled through a \mixing matrix, which dictates how agents average over their neighbors' parameter vectors. 
Thus, the \mixing matrix serves as a communication oracle which determines how information propagates throughout the network. 
Perhaps surprisingly, when the stepsizes are constant, simply averaging over the local iterates via the \mixing matrix only converges to a neighborhood of the optimum~\cite{yuan2016convergence,shi2015extra}.
% fails to yield a consensus among the agents~\cite{yuan2016convergence,shi2015extra}. 
% \mg{MG: There is actually consensus, all the iterates agree on a value but this value is $O(\alpha)$ away from the true optimizer. Consensus usually means that the nodes agree on a value..} \hz{Thanks for pointing this out, will change it.}
A recent line of works
\cite{shi2014linear, jakovetic2014linear, shi2015extra, qu2017harnessing, nedic2017achieving, nedic2017geometrically} 
proposed a number of alternative methods that linearly converge  to the global minimum. 
% proposed a number of alternative methods which are linearly convergent for smooth and strongly convex functions, reaching consensus asymptotically.

% Consequently, in a recent line of works
% \cite{shi2014linear, jakovetic2014linear, shi2015extra, qu2017harnessing, nedic2017achieving, nedic2017geometrically} proposed a number of alternative methods, leading to linear convergence rates for smooth and strongly convex local functions---in particular, a consensus is shown to hold asymptotically. 


The overall complexity of solving decentralized optimization problems is typically determined by two factors: (i) the condition number of the objective function $\kappa_f$, which measures the `hardness' of solving the underlying optimization problem, and (ii) the condition number of the mixing matrix $\kappa_W$, which quantifies the severity of information `bottlenecks' present in the network. Lower complexity bounds recently derived for distributed settings \cite{arjevani2015communication,scaman2017optimal,woodworth2018graph,arjevani2018tight} show that one cannot expect to have a better dependence on the condition numbers than  $\sqrt{\kappa_f}$ and  $\sqrt{\kappa_W}$. 
Notably, despite the considerable recent progress, none of the methods mentioned above is able to achieve accelerated rates, that is, a square root dependence for both ${\kappa_f}$ and ${\kappa_W}$---simultaneously.
%in addressing decentralized problems

An extensive effort has been devoted to obtaining acceleration for decentralized algorithms under various settings \cite{scaman2017optimal, scaman2018optimal,li2018sharp, xu2019accelerated, zhang2019achieving,uribe2020dual, hendrikx2020optimal,dvinskikh2019decentralized,fallah2019robust}. When a dual oracle is available, that is, access to the gradients of the dual functions is provided, optimal rates can be attained for smooth and strongly convex  objectives \cite{scaman2017optimal}.  However, 
having access to a dual oracle is a very restrictive assumption, and resorting to a direct `primalization' through inexact approximation of the dual gradients leads to sub-optimal  worst-case theoretical rates \cite{uribe2020dual}. In this work, we propose a novel primal approach that leads to optimal rates in terms of dependency on $\kappa_f$ and $\kappa_W$. 

% in this work we make the following contributions:
Our contributions can be summarized as follows.
\vspace{-0.2cm}
\begin{itemize}[leftmargin=.2in]
    \item We introduce a novel framework based on the accelerated augmented Lagrangian method for designing primal decentralized methods. The framework provides a simple and systematic way for deriving several well-known decentralized algorithms \cite{shi2014linear,jakovetic2014linear,shi2015extra}, including EXTRA~\cite{shi2015extra} and SSDA~\cite{scaman2017optimal}, and unifies their convergence analyses. 
    % \hz{it is not true that we could recover the EXTRA convergence result, need to find a rephrase}
    \item  Using accelerated gradient descent as a sub-routine, we derive a novel method
    for smooth and strongly convex local functions
    which achieves optimal \emph{accelerated} rates on both the condition numbers of the problem,  $\kappa_f$ and $\kappa_W$, using \emph{primal} updates, see~Table~\ref{tab:complexity}. 

    \item We perform a large number of experiments, which confirm our theoretical findings, and demonstrate a significant improvement when the objective function is ill-conditioned and $\kappa_f \gg \kappa_W$. 
\end{itemize}


==> [Neurips20] Decentralized Acc-AL algorithm /sections/sec2_setting.tex <==
\section{Decentralized Optimization Setting}
We consider $n$ computational agents and  a network graph $\G= (\mathcal{V}, \mathcal{E})$ which defines how the agents are linked. The set of vertices $\mathcal{V} = \{1, \cdots, n \}$ represents the agents and the set of edges $\mathcal{E} \in \mathcal{V} \times \mathcal{V}$ {specifies} {the} connectivity in the network, {i.e., a communication link between agents $i$ and $j$ exists if and only if $(i,j)\in\mathcal{E}$}. Each agent has access to  local information encoded by a loss function $f_i: \R^d \rightarrow \R$. The goal is to minimize the global {objective} over the entire network, 
\begin{equation}\label{eq:global}
	    \min_{x \in \R^d} f(x) \defeq \sum_{i=1}^n f_i(x).
	   % \vspace*{-0.1cm}
\end{equation} 
In this paper, we assume that the local loss functions $f_i$ are differentiable, $L$-smooth and $\mu$-strongly convex.\footnote{ \noindent $f$ is $L$-smooth if $\nabla f$ is $L$-Lipschitz; $f$ is $\mu$-strongly convex if $f-\frac{\mu}{2}\|x\|^2$ is convex.} {Strong convexity of the component functions $f_i$ implies that} the problem admits a unique solution, which we denote by $x^*$. 

We consider the following {computation and communication models}~\cite{scaman2017optimal}:
\vspace{-0.1cm}
\begin{itemize}[leftmargin=.2in]
    \item {\bf Local computation:} Each agent {is able to compute} the gradients of $f_i$ and the cost of this computation is one unit of time.
    % (a stronger assumption allows each agent to compute the gradients of the Fenchel conjugate function $f_i^*$)
    \item {\bf Communication:} Communication is done synchronously, and each agent {can} only exchange information with its neighbors, where $i$ is a neighbor of $j$ if $(i,j) \in \mathcal{E}$. The ratio between the communication cost and computation cost per round is denoted by $\tau$.
    % \yacomment{per round. Worth pointing out the synchronous nature of our computational model.}.
\end{itemize}
\vspace{-0.1cm}
% \yacomment{Below, large number of  distributed computational models do not fall under the category gossip model. Maybe `we assume' rather  `common'? It is a  definite (and fair) modeling choice.  }
% \begin{equation}\label{eq: local update}
%     x_i \leftarrow  \sum_{i =1}^n W_{ij} x_j. 
% \end{equation} 

% The exchange of information between the nodes is clearly determined by the properties of the mixing matrix $W$, 

We further assume that propagation of information is governed by a mixing matrix $W \in \R^{n \times n}$ \citep{nedic2009distributed, yuan2016convergence,scaman2017optimal}. Specifically, given a local copy of the decision variable $x_i \in \R^d$ at node $i\in[1,n]$, one round of communication provides the following update $x_i \leftarrow  \sum_{i =1}^n W_{ij} x_j$. The following 
% assumptions are standard  (see \cite{scaman2017optimal}.
standard assumptions regarding the mixing matrix \cite{scaman2017optimal} are made throughout the paper.
\begin{assumption}\label{ass:W}
The \mixing matrix $W$ satisfies the following:
\begin{enumerate}[leftmargin=.2in]
    \item {\bf Symmetry:} $W = W^T$.
    \item {\bf Positiveness:} $W$ is positive semi-definite.
    \item {\bf Decentralized property}: If $(i,j) \notin \mathcal{E}$ and $i \neq j$, then $W_{ij} = W_{ji} = 0$. 
    \item {\bf Spectrum property:} The kernel of $W$ is given by the vector of all ones $\mbox{Ker}(W)= \R \mathbf{1_n}$. \label{ass:W_spec}
\end{enumerate}
\end{assumption}
A typical choice of the mixing matrix is the (weighted) Laplacian matrix of the graph. Another common choice is to set $W$ as $I- \tilde{W}$ where $\tilde{W}$ is a doubly stochastic matrix \cite{aybat2017decentralized,can2019decentralized,shi2015extra}. By Assumption \ref{ass:W}.\ref{ass:W_spec}, all the eigenvalues of $W$ are strictly positive, except for the smallest one. We let  $\lambda_{\max}(W)$ denote the maximum eigenvalue, and let $\lambda_{\min}^+(W)$ denote the smallest positive eigenvalue.  The ratio between these two quantities plays an important role in quantifying the overall complexity of this problem.
% \yacomment{Should we also comment on the arbitrariness in the choice of $W$?}

% The decentralized property ensures that the exchange of information only occurs between neighbors; the doubly stochastic property ensures that the local update in (\ref{eq: local update}) acts as a weighted averaging; and, the symmetric property allows us to control the spectrum of $W$.
% \vspace{0.15cm}
% \begin{lemma}\label{prop-spectrum}
% Under Assumption~\ref{ass:W} and the connectivity of the graph $\G$, the spectrum of $W$ satisfies $1 = \lambda_1(W) > \lambda_2(W) \ge \cdots \ge \lambda_n(W) \ge -1.$
% Moreover, the top eigenspace of $W$ is the one-dimensional vector space spanned by the vector of all ones, i.e $\R \mathbf{1_n}$.
% \end{lemma}
% \mtodo{This is a well-known fact from the literature, should we state it as a lemma and give some refs?} \joan{well-known fact, chung book classic ref. }


% In particular, if we define $W_{neg} = I_n - W$, then $W_{neg}$ is positive semi-definite with null space $\mbox{Ker}(W_{neg}) = \R \mathbf{1_n}$. \joan{Why not denote it as a Laplacian?  } It turns out that the condition number of this matrix $W_{neg}$ plays an important role in the lower bounds {obtained in the literature as indicated by the following result}.
\vspace{0.15cm}
\begin{theorem}[Decentralized lower bound \cite{scaman2017optimal}] 
For any first-order black-box decentralized method, the number of time units required to reach an $\epsilon$-optimal solution for (\ref{eq:global}) is lower bounded by
\begin{equation}\label{eq:lower bound}
    \Omega \left ( \sqrt{\kappa_f} (1 + \tau \sqrt{\kappa_W} )  \log \left (\frac{1}{\epsilon} \right ) \right ),
\end{equation}
where $\kappa_f = L/\mu$ is the condition number of the loss function and $\kappa_W = \lambda_{\max}(W)/ \lambda^+_{\min}(W)$ is the condition number of  the \mixing matrix. 
\end{theorem}
The lower bound decomposes as follows: a) { \bf computation cost}, given by $\sqrt{\kappa_f} \log({1}/{\epsilon})$, and b) {\bf communication cost}, given by $\tau \sqrt{\kappa_f \kappa_W} \log({1}/{\epsilon})$.
%{In modern decentralized computation environments}\sout{real world setting}, the communication cost is {typically} \sout{usually} larger than the computation cost, i.e. $\tau \ge 1$ \cite{mcmahan2017communication}. In this case, the dominant term in the lower bound is  $O \left (\tau \sqrt{\kappa_f \kappa_W}  \log (\frac{1}{\epsilon}) \right )$. 
% look like $O\left ( \sqrt{\kappa_f }  \log (\frac{1}{\epsilon}) \right )$, that is in the decentralized setting, there is
The computation cost matches lower bounds for  centralized settings \cite{nesterov2004introductory,arjevani2016iteration}, while the communication cost introduces an additional term which depends on $\kappa_W$ and accounts for the `price' of communication in  decentralized models. It follows that the effective condition number of a given decentralized problem is  $\kappa_W{\kappa_f }$.

Clearly, the choice of the matrix $W$ can strongly affect the optimal attainable performance. For example, $\kappa_W$ can get as large as $n^2$ in the line/cycle graph, or be constant in the complete graph. 
In this paper, we do not focus on optimizing over the choice of $W$ for a given graph $G$; instead, following the approach taken by existing decentralized algorithms, we assume that the graph $G$ and
the mixing matrix W are given and aim to achieve the optimal complexity $\eqref{eq:lower bound}$ for this particular choice of $W$.
% In this paper, following the approach taken by existing state-of-the-art decentralized algorithms, we assume that the graph $\mathcal{G}$ and the \mixing matrix $W$ are given and aim to achieve the optimal complexity stated in {$\eqref{eq:lower bound}$ for this particular choice of $W$}.

% \joan{Perhaps it would be helpful to add a discussion on the tradeoffs faced when choosing $W$, even if these are not the focus of the contribution. Besides having $\bf{1}$ as leading eigenvector (implied by double stochastic), is the tradeoff between spectral gap (good rate) and sparsity (cheap computation)? Why is the restriction to a single $W$ a common choice? To what extent the relevant setup allows one to choose the topology rather than working from a given topology?}

% Before moving on we provide some canonical choice of the mixing matrix $W$. When the graph is $d$-regular, one could simply take $W = \frac{1}{d} A_{\G}$, where $A_{\G}$ is the adjacency matrix of~$\G$. For an arbitrary graph, one could {take}\sout{generalize it into} $W = I_n -  c \,\, {L_{\G}}$ where $ {L_{\G}}$ is the Laplacian matrix associated to the graph $\G$ and $c$ is a positive constant such that $c \le 1/\max d_i$, where $d_i$ is the degree of vertex $i$. We refer \yacomment{the reader} readers to section 2.4 in \cite{shi2015extra} for further examples.
 

==> [Neurips20] Decentralized Acc-AL algorithm /sections/sec3_related.tex <==
\section{Related Work and the Dual Formulation}
A standard approach to adress problem \eqref{eq:global} is to express it as a {constrained} optimization problem
\begin{equation}\label{primal}
\min_{\X \in \R^{nd}} %_{x_1=x_2= \cdots = x_n}  
F(\X):= \frac{1}{n} \sum_{i=1}^n f_i(x_i) \quad \mbox{such that} \quad x_1=x_2= \cdots = x_n \in \mathbb{R}^d\,, \tag{P}
\end{equation}
where $\X = [x_1;x_2; \cdots x_n] \in \R^{nd}$ is a concatenation of the vectors. 
To lighten the notation, we introduce the global mixing matrix $\W = W \otimes I_d \in \R^{nd \times nd}$, {where $\otimes$ denotes the Kronecker product}, and let $\| \cdot \|_{\W}$  denote the semi-norm induced by $\W$, i.e. $\|\X \|^2_{\W} = \X^T \W \X $. With this notation in hand, we briefly review existing literature on decentralized algorithms.
% \yacomment{To lighten notation? also the following notation is not used until in Section 3, so perhaps we can introduce it just before needed},
%Therefore, the update rule in (\ref{eq: local update}) is equivalent to the following matrix multiplication. \yacomment{Update rule (\ref{eq: local update}) now reads as follows:}
% \begin{equation} \label{eq: global update}
%     \X \leftarrow \W \cdot \X. 
% \end{equation} 



\paragraph{Decentralized Gradient Descent} The decentralized gradient method \cite{nedic2009distributed,yuan2016convergence} has the update rule
\begin{equation}
  \X_{k+1} = \W \X_k - \eta \nabla F(\X_k).  \tag{DGD}
\end{equation}
{However, with constant stepsize, the algorithm does not converge to a global minimum of \eqref{primal}, but rather to a neighborhood of the solution~\citep{yuan2016convergence}.} A decreasing stepsize schedule may be used to ensure convergence, but this yields a sublinear convergence rate, even in the strongly convex case.     

% \yacomment{Maybe, in terms of flow, first discuss primal algos and then motivate the introduction of the dual formulation by the optimality of SB? Should we also indicate at this point that the dual formulation is used extensively in the analysis?}

\begin{algorithm}[tb]
	\caption{Decentralized Augmented Lagrangian framework} \label{algo:AL}
	$\,\,$ {\bf Input:} mixing matrix $W$, regularization parameter $\rho$, stepsize $\eta$. \\
	\vspace{-0.4cm}
	\begin{algorithmic}[1]
		\FOR{$k = 1, 2, ..., K$} 
		\STATE $\X_{k} = \argmin  \left \{ P_k(\X) := F(\X) + \mathbf{\Lambda}_k^T \X +  \frac{\rho}{2}  \| \X \|^2_{\W}   \right \} $.
		  \STATE $\mathbf{\Lambda}_{k+1}  = \mathbf{\Lambda}_k + \eta \, \W \X_{k}$.
		\ENDFOR
	\end{algorithmic}
\end{algorithm}

\paragraph{Linearly convergent primal algorithms} 
% \yacomment{Recently, [] proposed the APM-C 
% algorithm which also enjoys a square root dependence on the condition number of the function and the graph. However, APM-C suffers an additional $\log(1/\epsilon)$ factor in terms of the computational(?) cost . In addition, our experiments indicate that our algorithm outperforms APM-C on various real-life problems.}
By and large,  recent methods that achieve linear convergence in the strongly convex case \cite{shi2014linear, jakovetic2014linear, shi2015extra, qu2017harnessing, nedic2017achieving, nedic2017geometrically,sun2019convergence} can be shown to follow a general framework based on the augmented Lagrangian method, see Algorithm~\ref{algo:AL}; The main difference lies in how subproblems $P_k$ are solved.   \citet{shi2014linear} apply an alternating directions method; in  \cite{shi2015extra}, the EXTRA algorithm takes a single gradient descent step to solve~$P_k$, see Appendix~B for details. \citet{jakovetic2014linear} use multi-step algorithms such as Jacobi/Gauss-Seidel methods. To the best of our knowledge, the complexity of these  algorithms is not better than  $O \left ((1+\tau) {\kappa_f \kappa_W}  \log (\frac{1}{\epsilon}) \right )$, in other words, they are non-accelerated. 
% {in the sense that the dependence is not of the order of $\sqrt{\kappa_f \kappa_W}$}.  
The recently proposed algorithm APM-C  \cite{li2018sharp} enjoys a square root dependence on $\kappa_f$ and $\kappa_W$, but incurs an additional $\log(1/\epsilon)$ factor compared to the optimal attainable rate.

\paragraph{Optimal method based on the dual formulation} 
By Assumption \ref{ass:W}.\ref{ass:W_spec}, the constraint $x_1=x_2= \cdots = x_n$ is equivalent to the identity $\W \cdot \X = 0 $, which is again equivalent to $\sqrt{\W} \cdot \X = 0$. Hence, the dual formulation of  \eqref{primal} is given by
\begin{equation}\label{dual}
    \max_{\mathbf{\Lambda} \in \mathbb{R}^{dn}} -F^*(- \sqrt{\W} \mathbf{\Lambda}).  \tag{D}
\end{equation} 
Since the primal function is convex and the constraints are linear, we can use strong duality and address the dual problem instead of the primal one. Using this approach, ~\cite{scaman2017optimal} proposed a dual method with optimal accelerated rates, using Nesterov's accelerated gradient method for the dual problem (\ref{dual}). As mentioned earlier, the main drawback of this method is that it requires access to the gradient of the dual function which, unless the primal function has a relatively simple structure, is not available. 
%and computing it exactly would be expensive \citn 
One may apply a first-order method to approximate the dual gradients inexactly at the expense of an additional $\sqrt{\kappa_f}$ factor in the computation cost~\cite{uribe2020dual}, but this woul make the algorithm no longer optimal. This indicates that achieving optimal rates when using primal updates is a rather challenging task in the decentralized setting. In the following sections, we provide a generic framework which allows us to derive a primal decentralized method with optimal complexity guarantees. 
%However, even though the communication cost remains unchanged, such inexact approach increases the computation cost by at least a factor of~$\sqrt{\kappa_f}$, introducing a gap compared to the optimal convergence rate~\cite{uribe2020dual}. 

%In other words, the algorithm is no longer with respect to the condition number $\kappa_f$ of the function. 
%this complexity result could be derived from our analysis and we will come back to it later in Section~{4}.

% Overall, deriving an optimal algorithm based on primal update is still an open question. Our approach closes this gap by introducing acceleration on the Augmented Lagrangian framework. 

% Linear convergent algorithms: \cite{shi2014linear, jakovetic2014linear, shi2015extra, qu2017harnessing, nedic2017geometrically}
% (see \cite{jakovetic2014linear, scaman2017optimal})

% Other optimal dual algorithms: \cite{uribe2020dual}

==> [Neurips20] Decentralized Acc-AL algorithm /sections/sec4_alg.tex <==
\section{An Inexact Accelerated Augmented Lagrangian framework}

\begin{algorithm}[tb]
	\caption{Accelerated Decentralized Augmented Lagrangian framework \label{algo:acc-AL}} 
		    {\bf Input:} mixing matrix $W$,  regularization parameter $\rho$, stepsize $\eta$, extrapolation parameters $\{\beta_k\}_{k \in \N}$ \\
	\vspace{-0.4cm}
	\begin{algorithmic}[1]
	    \STATE Initialize dual variables $\mathbf{\Lambda}_1 =\mathbf{\Omega}_1 =\mathbf{0} \in \R^{nd}$.
		\FOR{$k = 1, 2, ..., K$} 
		\STATE $\X_{k} = \argmin  \left \{ P_k(\X) := F(\X) + \mathbf{\Omega}_k^T \X +  \frac{\rho}{2}  \| \X \|^2_{\W}   \right \} $.
		  \STATE $\mathbf{\Lambda}_{k+1}  = \mathbf{\Omega}_k + \eta \W \X_{k}$
		  \STATE $\mathbf{\Omega}_{k+1} =  \mathbf{\Lambda}_{k+1} + \beta_{k+1} (\mathbf{\Lambda}_{k+1} - \mathbf{\Lambda}_k) $
		\ENDFOR
	\end{algorithmic}
	{\bf Output: $\X_K$.} 
\end{algorithm}
\begin{algorithm}[tb]
	\caption{\our : Inexact Acc-Decentralized Augmented Lagrangian framework \label{algo:inexact acc-AL}} 
	{\bf Additional Input:} A first-order optimization algorithm $\mathcal{A}$ \\
	Apply $\mathcal{A}$ to solve the subproblem $P_k$ warm starting at $\X_{k-1}$ to find an approximate solution
    \[\X_{k} \approx \argmin  \left \{ P_k(\X) := F(\X) + \mathbf{\Omega}_k^T \X +  \frac{\rho}{2}  \| \X \|^2_{\W}   \right \} ,\]
    \begin{description}
    \item[Option I:] stop the algorithm when $ \| \X_k - \X_k^*\|^2 \le \epsilon_k$, where $\X_k^*$ is the unique minimizer of $P_k$.
    \item[Option II:] stop the algorithm after a prefixed number of iterations $T_k$.
    \end{description}
\end{algorithm}

% \joan{Matrix norms $\| X \|_{W_{neg}}^2$ not introduced (as an aside, this is known as the Dirchlet energy) }

In this section, we introduce our inexact accelerated Augmented Lagrangian framework, and show how to combine it with Nesterov's acceleration. To ease the presentation, we first describe a conceptual algorithm, Algorithm \ref{algo:acc-AL}, where subproblems are solved exactly, and only then introduce inexact inner-solvers. 

Similarly to Nesterov's accelerated gradient method, we use  an extrapolation step for the dual variable~$\mathbf{\Lambda}_{k}$. The component $\W \X_k$ in line~4 of Algorithm~\ref{algo:acc-AL} is the negative gradient of the Moreau-envelope\footnote{A proper definition of the Moreau-envelope is given in \cite{rockafellar2009variational}, readers that are not familiar with this concept could take it as an implicit function which shares the same optimum as the original function.} of the dual function. Hence our algorithm is equivalent to applying Nesterov's method on the Moreau-envelope of the dual function, or equivalently, an accelerated dual proximal point algorithm. This renders the optimal dual method proposed in~\cite{scaman2017optimal} as a special case of our algorithmic framework (with $\rho$ set to 0). %The recent primal-dual accelerated method in~\cite{xu2019accelerated} can also be interpreted as a special case of our algorithm, by using accelerated gradient descent as a subroutine. 
% These connections make our framework because of the unified viewpoint on existing methods.

% This connection makes our analysis generalizable to an inexact variant of~\cite{scaman2017optimal}.

While Algorithm~\ref{algo:acc-AL} is conceptually plausible, it requires an exact solution of the Augmented Lagrangian problems, which can be too expensive in practice. To address this issue, we introduce an inexact version, shown in Algorithm~\ref{algo:inexact acc-AL}, where the $k$-th subproblem $P_k$ is solved up to a predefined accuracy~$\epsilon_k$. The choice of $\epsilon_k$ is rather subtle. On the one hand, choosing a large $\epsilon_k$ may result in a non-converging algorithm. On the other hand,  choosing a small $\epsilon_k$ can be exceedingly expensive as the optimal solution of the subproblem $\X_k^*$ is not the global optimum~$\X^*$.  Intuitively, $\epsilon_k$ should be chosen to be of the same order of magnitude as $\| \X_k^* -\X^*\|$, leading  to the following result.

% One of our main contributions lies in carefully leveraging the inexactness and evaluating the necessary complexity for solving the subproblem.   
% \mtodo{Last sentence was not entirely clear to me, can we rewrite it?}

\begin{theorem}\label{thm:main}
Consider the sequence of primal variables $(\X_k)_{k \in \N}$ generated by Algorithm~\ref{algo:inexact acc-AL} with the subproblem $P_k$ solved up to $\epsilon_k$ accuracy in Option~I. With parameters set to
\begin{equation}
    \beta_k = \frac{\sqrt{L_\rho} - \sqrt{\mu_\rho}}{ \sqrt{L_\rho}+\sqrt{\mu_\rho}}, \quad \eta = \frac{1}{L_\rho}, \quad \epsilon_k = \frac{\mu_\rho}{2 \lambda_{\max}(W)} \left (1-\frac{1}{2}\sqrt{\frac{\mu_\rho}{L_\rho}} \right )^k \Delta_{dual},
\end{equation}
where $L_\rho = \frac{\lambda_{\max}(W)}{\mu + \rho \lambda_{\max}(W) }$, $\mu_\rho = \frac{\lambda_{\min}^+(W)}{L + \rho \lambda_{\min}^+(W)}$ and $\Delta_{dual}$ is the initial dual function gap, we obtain 
\begin{equation}
     \| \X_{k} - \X^* \|^2 \le C_\rho \left ( 1- \frac{1}{2} \sqrt{\frac{\mu_\rho}{L_\rho}}\right )^{k} \Delta_{dual},
\end{equation}
where $\X^*=\mathbf{1}_n \otimes x^*$ and $C_\rho = 258 \frac{L_\rho \lambda_{\max}(W) }{\mu^2 \mu_\rho^2}$.
\end{theorem}
\begin{corollary}
The number of subproblems $P_k$ to achieve $\| \X_k - \X^* \|^2 \le \epsilon$ in \our~is bounded by 
\begin{equation}\label{eq: outer iteration}
    K= O\left( \sqrt{\frac{L_\rho}{\mu_\rho}} \log \left(\frac{C_\rho \Delta_{dual}}{\epsilon} \right )\right).
\end{equation}
\end{corollary}
We remark that inexact accelerated Augmented Lagrangian methods have been previously analyzed  under different assumptions \cite{nedelcu2014computational, kang2015inexact,yan2020bregman}. The main difference is that here, we are able to establish a linear convergence rate, whereas existing analyses only yield sublinear  rates. One of the reasons for this discrepancy is that, although $F^*$ is strongly convex, the dual problem (\ref{dual}) is not, as the mixing matrix $\W$ is singular.  The key to obtaining a linear convergence rate is a fine-grained analysis of the dual problem, showing that the dual variables always lie in the subspace where strong convexity holds. The proof of the theorem relies on the equivalence between Augmented Lagrangian methods and the dual proximal point algorithm \cite{rockafellar1976augmented,bertsekas2014constrained}, which can be interpreted as applying an inexact accelerated proximal point algorithm \cite{guler1992new, lin2017catalyst} to the dual problem. A complete convergence analysis is deferred to Section~C in the appendix.  
% The strong convexity only holds in the image space of $\W$. 
%~\ref{app:proof of main thm}



% We remark that even though $F^*$ is strongly convex, the dual problem (\ref{dual}) is not, since $\W$ is singular. Thus, in order to obtain a linear convergence rate, we need to show that the dual iterates lie in the image space of $\W$ where the function is strongly convex \cite{jakovetic2014linear,scaman2017optimal}.

%in the primal iterates
{Theorem \ref{thm:main} provides} an accelerated convergence rate with respect to the `augmented' condition number {$\kappa_\rho:=L_\rho/\mu_\rho$, as determined by the Augmented Lagrangian parameter~$\rho$ in Algorithm~\ref{algo:inexact acc-AL}. We have the following bounds:}
\begin{equation}\label{eq:aug condition number}
  \underbrace{1}_{\rho = \infty} \le %\frac{L_\rho}{\mu_\rho} 
  \kappa_\rho= \frac{L+\rho \lambda_{\min}^+(W) }{\mu + \rho \lambda_{\max}(W)} \frac{\lambda_{\max}(W)}{\lambda_{\min}^+(W)}  \le \underbrace{\frac{L}{\mu} \frac{\lambda_{\max}(W)}{\lambda_{\min}^+(W)}}_{\rho =0} = \kappa_f \kappa_W,
\end{equation}
%which is determined by the Augmented Lagrangian parameter~$\rho$. 
%In particular, 
where we observe that the condition number $\kappa_\rho$ is a decreasing function  of the regularization parameter~$\rho$. When $\rho =0$, the maximum value is attained at $\kappa_\rho=\kappa_f \kappa_W$,  the effective condition number of the decentralized problem. As $\rho$ goes to infinity, the augmented condition number $\kappa_\rho$ {goes to 1}. Naively, one may want to take $\rho$ as large as possible to get a fast convergence. However, one must also take into account the complexity of solving the subproblems. Indeed, since $W$ is singular, the additional regularization term in $P_k$ does not improve the strong convexity of the subproblems, yielding an increase in inner {loops} complexity as $\rho$ grows.
% , whcih  increasing the complexity of the inner {loops} as $\rho$ grows. 
Hence, the optimal choice of~$\rho$ requires balancing {the inner and outer complexity in a careful manner}.
%computational complexity of the inner {loop} increases as $\rho$ grows.
% \yacomment{Perhaps it's better not to have two tables at the top of the same page...}

%have not yet taken the complexity of the subproblems into account. Indeed, the computational complexity in the inner \mg{loop} increases as $\rho$ grows. Hence the optimal choice of $\rho$ requires balancing \mg{the inner and outer complexity in a careful manner}.  
% \yacomment{Should further emphasize the inability of solving  $\rho=0$ exactly, unless a dual oracle is given.}

% Intuitively, in order to guarantee a similar convergence rate as the exact algorithm, the inexactness of the gradient should be at the same magnitude as the suboptimality $\| X_k -X^*\|^2$. This is exactly the corollary is stating. In particular, this provides the number of outer loop iterations, i.e. update on the dual variables. We remark that the condition number $L_\rho/\mu_\rho$ improves as $\rho$ increases. More precisely,
% \[  \underbrace{1}_{\rho = \infty} \le \frac{L_\rho}{\mu_\rho} \le \underbrace{\frac{L}{\mu} \frac{1-\lambda_n(W)}{1-\lambda_2(W)}}_{\rho =0} = \kappa_f \kappa_W  \]
%This is why adding the Augmented Lagrangian component helpful since it helps improving the condition number of the Moreau-envelope. 
%The optimal choice of $\rho$ is to take $\rho = \frac{L}{1-\lambda_n(W)}$, in which case,
%\[  \frac{L_\rho}{\mu_\rho} \le  2 \frac{1-\lambda_n(W)}{1-\lambda_2(W)} \]
%which does not depend on the condition number of the function $\kappa_f$. 


   
To study the inner loop complexity, we introduce a warm-start strategy.
% for the $k$-th iteration at $\X_{k-1}$.
Intuitively, the distance between $\X_{k-1}$ and the $k$-th {solution }$\X_k^*$ {to the subproblem $P_k$} is roughly  {on the} order of $\epsilon_{k-1}$. 
More precisely, we have the following result.
\begin{lemma}\label{lemma:inner}
Given the parameter choice in Theorem~\ref{thm:main}, initializing the subproblem $P_k$ at $\X_{k-1}$ yields,
% With the parameter choice as {given in} Theorem~\ref{thm:main}, if the subproblem $P_k$ are initialized at $X_{k-1}$, then 
% \mg{if subproblem $P_k$ is solved with initialization $X_{k-1}$, then the solution $X_k^*$ satisfies} 
%\mg{if subproblem $P_k$ is solved with initialization $X_{k-1}$, then the solution $X_k^*$ satisfies} 
\[ \| \X_{k-1} - \X_k^*\|^2  \le \frac{8 C_\rho}{\mu_\rho} \epsilon_{k-1}.  \]
\end{lemma}

 \newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
\begin{table*}\centering 
\ra{1.3}
\begin{tabular}{@{}lcrcrc@{}}\toprule
& {GD} & \phantom{abc}& {AGD} &
\phantom{abc} & {SGD}\\ \midrule
%Inner loop complexity $T_k$ & 0.0790  && 0.3670  && -1.0032 \\
% {SSDA+GD} 
% & 0  && $\tilde{O} \left( \kappa_f \right )$ &&  $O\left ((\kappa_f+\tau)  \sqrt{\kappa_f \kappa_W} log(\frac{1}{\epsilon}) \right)$ \\
% \our+GD & $\frac{L}{\lambda_1(W)}$  && $\tilde{O} \left( \kappa_f \right )$ &&  $O\left ((1+\tau) \kappa_f \sqrt{\kappa_W} \log(\frac{1}{\epsilon}) \right)$ \\
 {$T_k$} 
& $\tilde{O}\left ( \frac{L + \rho \lambda_{\max}(W)}{\mu}  \right )$    && $\tilde{O}\left ( \sqrt{\frac{L + \rho \lambda_{\max}(W)}{\mu}}  \right )$  &&  $\tilde{O} \left (  \frac{\sigma^2}{\mu^2 \epsilon_k}  \right)$ \\
 {$\rho$} & $\frac{L}{\lambda_{\max}(W)}$    &&  $\frac{L}{\lambda_{\max}(W)}$  &&   $\frac{L}{\lambda^+_{\min}(W)}$ \\
 {$\displaystyle   \sum_{k=1}^K T_k$} & $\tilde{O}\left ( \kappa_f \sqrt{\kappa_W} \log(\frac{1}{\epsilon})   \right )$    && $\tilde{O}\left (  \sqrt{\kappa_f \kappa_W} \log(\frac{1}{\epsilon})   \right )$  &&  $\tilde{O} \left (\frac{\sigma^2 \kappa_f \kappa_W}{\mu^2 \epsilon} \right)$ \\
\bottomrule
\end{tabular}
\caption{The first row indicates the number of iterations required for different inner solvers to achieve~$\epsilon_k$ accuracy for the $k$-th subproblem $P_k$; the $\tilde{O}$ notation hides logarithmic factors in the parameters $\rho$, $\kappa_f$ and  $\kappa_W$. The second row shows the theoretical choice of the regularization parameter $\rho$. The last row shows the
total number of iterations according to the choice of $\rho$. }\label{tab:inner complexity}
\end{table*}


%\joan{perhaps give a more explicit dependency of this ratio in terms of $\rho$?} 
 Consequently, the ratio between the initial gap at the $k$-th subproblem and the desired gap $\epsilon_k$ is bounded by
 \[ \frac{\| \X_{k-1} - \X_k^*\|^2 }{\epsilon_k} \le  \frac{8 C_\rho}{\mu_\rho} \frac{\epsilon_{k-1}}{\epsilon_k} \le \frac{16 C_\rho}{\mu_\rho} = O(\kappa_f \kappa_W \rho^2),\]
 which is  independent of $k$. In other words, the inner loop solver only needs to decrease the iterate gap by a constant factor for each $P_k$. If the algorithm enjoys a linear convergence rate, a constant number of iteration is sufficient for that. If the algorithm enjoys a sublinear convergence, then the inner loop complexity grows with~$k$. To illustrate the behaviour of different algorithms, we present the inner loop complexity $T_k$ for gradient descent (GD), accelerated gradient descent (AGD) and stochastic gradient descent (SGD) in Table~\ref{tab:inner complexity}. Note that while the inner complexity  of GD and AGD are independent of $k$, the inner complexity for SGD increases geometrically with $k$. Other possible choices for inner solvers are the alternating directions or Jacobi/Gauss-Seidel method, both of which yield accelerated variants for  \cite{shi2014linear} and \cite{jakovetic2014linear}.
 
% \yacomment{GD, AGD abbreviations should be presented at earlier stages}
 
 In fact, the theoretical upper bounds on the inner complexity also provide a more practical way to halt the inner optimization processes (see Option II in Algorithm~\ref{algo:inexact acc-AL}). Indeed, one can  predefine the computational budget for each subproblem, for instance, $100$ iterations of AGD. If this budget exceeds the theoretical inner complexity $T_k$ in Table~\ref{tab:inner complexity}, then the desired accuracy~$\epsilon_k$ is guaranteed to be reached. In particular, we do not need to evaluate the sub-optimality condition, it is automatically satisfied as long as the budget is chosen appropriately. 
 
 
%  by running $T_k$ iterations of the given inner solver, the desired accuracy $\epsilon_k$ can also be reached. In other words, we do not need to evaluate the sub-optimality condition, rather it is automatically satisfied as long as $T_k$ is chosen properly. 
%  \yacomment{Paragraph above can be further clarified I feel}
 
% \begin{itemize}[leftmargin=.2in]
%     \item {\bf GD}: when applying gradient descent as inner solver, the inner loop complexity is given by 
%     \[ T_k = O\left ( \frac{L + \rho \lambda_1(W)}{\mu}  \log \left ( C \frac{\epsilon_{k-1}}{\epsilon_k} \right ) \right )\]
%     \item {\bf AGD}: when applying accelerated gradient descent as inner solver, the inner loop complexity is given by 
%     \[ T_k = O\left ( \sqrt{\frac{L + \rho \lambda_1(W)}{\mu}}  \log( 8\frac{C_\rho}{\mu_\rho} \frac{\epsilon_{k-1}}{\epsilon_k} )\right ) \]
%     \item {\bf SGD}: when applying stochastic gradient descent as inner solver, the inner loop complexity is given by 
%     \[ T_k =\]
% \end{itemize}


Finally, the global complexity is obtained by summing $\sum_{k=1}^K T_k$, where $K$ is the number of subproblems given in (\ref{eq: outer iteration}). Note that, so far, our analysis applies to any regularization parameter~$\rho$. Since $\sum_{k=1}^K T_k$ is a function of $\rho$, this implies that one can select the parameter $\rho$ such that the overall  complexity is minimized, leading to the choices of $\rho$ described in Table~\ref{tab:inner complexity}.

\paragraph{Two-fold acceleration} In our setting, acceleration seems to occur in two stages (when compared to the non-accelerated  $O\left ( \kappa_f {\kappa_W} \log(\frac{1}{\epsilon})   \right )$ rates in \cite{shi2014linear, jakovetic2014linear, shi2015extra, qu2017harnessing, nedic2017achieving}). First, combining \our~with GD improves the dependence on the condition of the  mixing matrix $\kappa_W$. Secondly, when used as an inner solver, AGD  improves the dependence on  the condition number of the local  functions $\kappa_f$. This suggests that the two phenomena are independent; while one is related to the consensus between the agents, as governed by the mixing matrix, the other one is related to the respective centralized hardness of the optimization problem. 


\paragraph{Stochastic oracle} Our framework also subsumes the stochastic setting, where only noisy gradients are available. In this case, since SGD is  sublinear, the required iteration counters $T_k$ for the subproblem must increase inversely proportional to~$\epsilon_k$. Also the stepsize at the $k$-th iteration needs to be decreased accordingly. The overall complexity is now given by $\tilde{O} \left (\frac{\sigma^2 \kappa_f \kappa_W}{\mu^2 \epsilon} \right)$. 
However, in this case, the resulting dependence on the graph condition number can be improved \cite{fallah2019robust}.


% This phenomenon does not occur in the Catalyst framework~\cite{lin2017catalyst} where applying GD already achieves the optimal convergence rate. In other words, the acceleration is two-folded: a) the acceleration on the dual variable gains $\sqrt{\kappa_W}$; b) the acceleration in the inner loop gains $\sqrt{\kappa_f}$. We remark that here we are interested in the setting $\tau \ge 1$, i.e. communication cost is higher than computation cost. In the fast communication scenario, one need to incorporate the multi-stage procedure as in \cite{scaman2017optimal}. We leave the proper derivation as a future direction. 
% \yacomment{Maybe name the paragraph as 'Two-fold acceleration'? Also, needs to better explain why the Catalyst framework is referred to here, i.e., a *centralized* iterative procedure of inexactly solving 'warm-started' sub-problems.}



\paragraph{Multi-stage variant (M\our)} We remark that the complexity presented in Table~\ref{tab:complexity} is abbreviated, in the sense that it does not distinguish between communication cost and computation cost. To provide a more fine-grained analysis, it suffices to note that performing a gradient step of the subproblem $\nabla P_k(\X)= \nabla F(\X) + \mathbf{\Omega}_k + \rho \W \X  $ requires one local computation to evaluate $\nabla F$,  and one round of communication to obtain $\W \X$. This implies that when  GD/AGD/SGD is combined with \our, the number of local computation rounds is roughly the number of communication rounds, leading to a sub-optimal computation cost, as shown in Table~\ref{tab:complexity}.

% Note that performing a gradient step of $\nabla P_k(\X)= \nabla F(\X) + \mathbf{\Omega}_k + \rho \W \X  $ requires one local computation to evaluate $\nabla F$,  and one round of communication to obtain $\W \X$. This implies that  the number of local computation round is roughly equal to the number of communication round, leading to a sub-optimal computation cost as shown in~Table~\ref{tab:complexity}. 
To achieve optimal accelerated rates, we enforce multiple communication rounds after one evaluation of $\nabla F$. This is achieved by substituting the regularization metric $\| \cdot \|^2_\W$ with $\| \cdot \|^2_{Q(\W)}$, where $Q$ is a well-chosen polynomial. In this case, the gradient of the subproblem becomes $\nabla P_k(\X)= \nabla F(\X) + \mathbf{\Omega}_k + \rho \,\, Q(\W) \X $, which requires $\deg(Q)$ rounds of communication.

% Note that performing a gradient step of $\nabla P_k(\X)= \nabla F(\X) + \mathbf{\Omega}_k + \rho \W \X  $ requires one local computation to evaluate $\nabla F$,  and one round of communication to obtain $\W \X$. This implies that  the number of local computation round is roughly equal to the number of communication round, leading to a sub-optimal computation cost as shown in~Table~\ref{tab:complexity}. In order to achieve optimal accelerated rates, we enforce multiple communication rounds after one evaluation of $\nabla F$ by substituting the regularization metric $\| \cdot \|^2_\W$ with $\| \cdot \|^2_{Q(\W)}$, where $Q$ is a well-chosen polynomial. In particular, the gradient of the subproblem becomes $\nabla P_k(\X)= \nabla F(\X) + \mathbf{\Omega}_k + \rho \,\, Q(\W) \X $, which requires $\deg(Q)$ rounds of communication.



The choice of the polynomial $Q$ relies on Chebyshev acceleration, which is  introduced in~\cite{ scaman2017optimal,lecturenote}.  More concretely, the Chebyshev polynomials are defined by the recursion relation $T_0(x)=1$, $T_1(x) =x$, $T_{j+1}(x) = 2x T_j(x) - T_{j-1}(x)$, and $Q$ is defined by
\begin{equation}\label{eq:Q}
    Q(x) = 1- \frac{T_{j_W}(c(1-x))}{T_{j_W}(c)} \quad \text{ with } \quad j_W = \lfloor \sqrt{\kappa_W} \rfloor, \quad  c= \frac{\kappa_W +1}{\kappa_W-1}.
\end{equation}
Applying this specific choice of $Q$ to the mixing matrix $W$ reduces its condition number by the maximum amount \cite{ scaman2017optimal,lecturenote}, yielding a graph independent bound $\kappa_{Q(W)} = \lambda_{\max}(Q(W))/ \lambda^+_{\min}(Q(W)) \le4$. Moreover, the symmetry, positiveness and spectrum property in Assumption~\ref{ass:W} are maintained by~$Q(W)$.
% Applying this specific choice of $Q$ to the mixing matrix $W$ maintains the symmetry, positiveness and spectrum property in Assumption~\ref{ass:W}, and improves the effective condition number by $\kappa_{Q(W)} = \lambda_{\max}(Q(W))/ \lambda^+_{\min}(Q(W)) \le 4$.  
Even though $Q(W)$ no longer satisfies the decentralized property, it can be implemented using $\lfloor \sqrt{\kappa_W} \rfloor$ rounds of communications with respect to~$W$. The implementation details of the resulting algorithm are similar to Algorithm~\ref{algo:acc-AL}, and follow by substituting the mixing matrix $W$ by~$Q(W)$ (Algorithm~5 in  Appendix~E).%\ref{appendix: mideal})

% Conceptually, this could be interpreted as substituting the mixing matrix $W$ to $Q(W)$.

% This is equivalent to replacing the mixing matrix $\W$ by a polynomial of it. This could be achieved by applying the multi-stage technique introduced in~\cite{scaman2017optimal}, based on Chebyshev acceleration. 



%replace the augmented regularizer $\| \cdot \|^2_\W$ in the subproblems by $\| \cdot \|^2_{Q_{\sqrt{\kappa_W}}(\W)}$ where $Q$ is a polynomial given by

%where $T_j$ are the Chebyshev polynomials defined by recursion $T_0(x)=1$, $T_1(x) =x$ and $T_{j+1}(x) = 2x T_j(x) - T_{j-1}(x)$. 



% the mixing matrix $\W$ shows up in the subproblems formulation of $P_k$, as a matrix regularizer, this means running GD/AGD/SGD in the inner problem requires communication. Hence the number of communication round is the same as the number of local computation shown in the last row in Table~\ref{tab:inner complexity}, yielding a non optimal communication cost.  This could be achieved by applying the multi-stage technique introduced in~\cite{scaman2017optimal}, based on Chebyshev acceleration. 
% More precisely, we replace the augmented regularizer $\| \cdot \|^2_\W$ by $\| \cdot \|^2_{Q(\W)}$ where $Q$ is a polynomial given by
% \begin{equation}
%     Q_j(x) = 1- \frac{T_j(c(1-x))}{T_j(c)} \quad \text{ with } \quad c= \frac{\kappa_W +1}{\kappa_W-1}.
% \end{equation}
% where  and $T_K$ are the Chebyshev polynomials. 

% multiple rounds of communications. We combine the Chebyshev acceleration technique introduced in \cite{scaman2017optimal}. The only changes in the our algorithm is to replace the matrix $W$ by $Q_k(W)$ where $Q_k$ is determined by


\begin{table*}\centering 
\ra{1.3}
\begin{tabular}{@{}lcrcrc@{}}\toprule
& {$\rho$} & \phantom{abc}& {Computation cost} &
\phantom{abc} & {Communication cost}\\ \midrule
%Inner loop complexity $T_k$ & 0.0790  && 0.3670  && -1.0032 \\
% {SSDA+GD} 
% & 0  && $\tilde{O} \left( \kappa_f \right )$ &&  $O\left ((\kappa_f+\tau)  \sqrt{\kappa_f \kappa_W} log(\frac{1}{\epsilon}) \right)$ \\
% \our+GD & $\frac{L}{\lambda_1(W)}$  && $\tilde{O} \left( \kappa_f \right )$ &&  $O\left ((1+\tau) \kappa_f \sqrt{\kappa_W} \log(\frac{1}{\epsilon}) \right)$ \\
 {SSDA+AGD} 
& 0   && $\tilde{O} \left (\kappa_f \sqrt{\kappa_W} \log(\frac{1}{\epsilon}) \right)$ &&  $O\left ( \tau  \sqrt{\kappa_f  \kappa_W} \log(\frac{1}{\epsilon}) \right)$ \\
{\our+AGD} & $\frac{L}{\lambda_{\max}(W)}$   && $\tilde{O} \left( \sqrt{\kappa_f \kappa_W} \right ) \log(\frac{1}{\epsilon})$ &&  $ \tilde{O} \left (\tau   \sqrt{\kappa_f \kappa_W} \log(\frac{1}{\epsilon}) \right)$ \\
 {MSDA+AGD} 
& 0   &&  $\tilde{O} \left (\kappa_f \log(\frac{1}{\epsilon}) \right)$ &&  $O\left ( \tau   \sqrt{\kappa_f  \kappa_W} \log(\frac{1}{\epsilon}) \right)$ \\
{M\our+AGD} & $\frac{L}{\lambda_{\max}(Q(W))}$   && $\tilde{O} \left( \sqrt{\kappa_f} \log(\frac{1}{\epsilon}) \right )$ &&  $\tilde{O} \left ( \tau \sqrt{\kappa_f \kappa_W} \log(\frac{1}{\epsilon}) \right)$ \\
%\our+SGD &  $\frac{L}{1-\lambda_n(W)}$ && $O\left(\right )$ && $O\left ( \right)$ \\

\bottomrule
\end{tabular}
\caption{ The communication cost of the presented algorithms are all optimal, but the computation cost differs. An additional factor of $\sqrt{\kappa_f}$ is introduced in SSDA/MSDA compared to their original rate in~\cite{scaman2017optimal}, due to the gradient approximation. The optimal computation cost is achieved by combining our multi-stage algorithm MIDEAL with AGD as an inner solver. 
 }\label{tab:complexity}
 % The computation cost of SSDA~\cite{scaman2017optimal} increases when the gradient of the dual function need to be solved inexactly. By applying our framework~\our, we recover the complexity of exact SSDA~\cite{scaman2017optimal}. To further accelerate the computation cost, an additional multi-stage technique similar to~\cite{scaman2017optimal} needs to be deployed. We named it by MIDEAL, which achieves the optimal computation and communication rate.
% \yacomment{MIDEAL should be assumed known at this the stage.}
% The inexact variant of~\cite{scaman2017optimal}, by applying the AGD solver to inexactly approximate the gradient of the dual function does not yield the optimal computation cost. 
\end{table*}


\paragraph{Comparison with inexact SSDA/MSDA \cite{scaman2017optimal}} Recall that SSDA/MSDA are special cases of our algorithmic framework
with the degenerate regularization parameter $\rho=0$. 
% , and follow by setting  the  regularization parameter $\rho$ to 0.
Therefore, our complexity analysis naturally extends to an inexact anlysis of SSDA/MSDA, as shown in Table~\ref{tab:complexity}. although the resulting communication costs are optimal,  the computation cost is not, due to the additional $\sqrt{\kappa_f}$ factor  introduced by solving the subproblems inexactly. In contrast, our multi-stage framework achieves the optimal computation cost. 
\begin{itemize}[leftmargin=.1in]
    \item {\bf Low communication cost regime: $\tau \sqrt{\kappa_W}<1$}, the computation cost dominates the communication cost, a $\sqrt{\kappa_f}$ improvement is obtained by MIDEAL comparing to MSDA. 
    \item {\bf Ill conditioned regime: $1 < \tau \sqrt{\kappa_W}< \sqrt{\kappa_f}$}, the complexity of MSDA is dominated by the computation cost $\tilde{O} \left (\kappa_f \log(\frac{1}{\epsilon}) \right)$ while the complexity MIDEAL is dominated by the communication cost $\tilde{O} \left (\tau \sqrt{\kappa_f \kappa_W} \log(\frac{1}{\epsilon}) \right)$. The improvement is proportional to the ratio $\sqrt{\kappa_f}/\tau \sqrt{\kappa_W}$.
    \item {\bf High communication cost regime: $\sqrt{\kappa_f}<\tau \sqrt{\kappa_W}$}, the communication cost dominates, and MIDEAL and MSDA are comparable.
\end{itemize}

% As noted earlier, the overall complexity is the sum of 
% %consists of 
% computation cost and the communication cost. The regime that our algorithm 

% When the problem is ill-conditioned to the extent where $\sqrt{\kappa_f} > \tau \sqrt{\kappa_W}$, our framework outperforms inexact MSDA. Otherwise, when the communication cost dominates, both convergence rates are of the same order.  

%We remark that the naive approach to inexactly approximate the gradient of dual function does not lead to an optimal convergence rate.


% Indeed, our framework recovers SSDA by setting the regularization parameter $\rho=0$. Based on the convergence analysis, the global complexity of inexact SSDA
% and MSDA are given by $O\left ((\sqrt{\kappa_f}+\tau)  \sqrt{\kappa_f  \kappa_W} log(\frac{1}{\epsilon}) \right)$ and $O\left ((\kappa_f+\tau  \sqrt{\kappa_f  \kappa_W} ) log(\frac{1}{\epsilon}) \right)$. 

% \yacomment{commenting in someone else's comment: Discuss that $\|\X_k -\X^* \|$ could not be evaluated but  instead we could predefine the $T_k$. }


% \newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}





% \paragraph{Comparison with inexact SSDA/MSDA \cite{scaman2017optimal}} 

% is $O\left ((1+\tau)  \kappa_f^{3/2} \sqrt{\kappa_W} log(\frac{1}{\epsilon}) \right)$ and $O\left ((1+\tau)  \kappa_f \sqrt{\kappa_W} log(\frac{1}{\epsilon}) \right)$ when solved by GD and AGD, respectively. The reason that taking $\rho=0$ is not a good idea is because the augmented condition number in (\ref{eq:aug condition number}) maximizes when $\rho =0$. When we use the suggested choice $\rho = \frac{L}{1-\lambda_n(W)}$, this condition number is $2 \kappa_W$, which is independent of $\kappa_f$.















% It is well known that Augmented Lagrangian method is equivalent to apply the proximal point algorithm on the dual problem  \cite{rockafellar1976augmented, bertsekas2014constrained}, which is again equivalent to gradient descent on the Moreau-envelope of the dual problem.






% \paragraph{Sketch of the proof} Inexact proximal point algorithm \cite{schmidt2011convergence,lin2017catalyst}

% We define the Moreau-envelope of the dual problem (\ref{dual}): 
% \begin{equation}
%     \Phi_\rho(\Lambda) =  \min_{\Gamma \in \R^{nd}} \left \{  F^*(-\sqrt{W_{neg}} \Gamma ) + \frac{1}{2\rho} \| \Gamma -\Lambda\|^2 \right \}
% \end{equation}
% \begin{proposition}
% The Moreau envelope $\Phi_\rho$ enjoys the following properties 
% \begin{itemize}
%     \item $\Phi_\rho$ is convex, differentiable and $\Phi_\rho$ shares the same optimum as the dual problem (\ref{dual}).
%     \item $\Phi_\rho$ is $L_\rho$-smooth, where $L_\rho = \frac{1-\lambda_n(W)}{\mu + \rho (1-\lambda_n(W))} \le \frac{1}{\rho}$.
%     \item $\Phi_\rho$ is $\mu_\rho$-strongly convex in the image space of $\sqrt{W_{neg}}$, where $\mu_\rho = \frac{1-\lambda_2(W)}{L + \rho (1-\lambda_2(W))}$.
% \end{itemize}
% \end{proposition}
% More importantly,  the optimum of the Augmented Lagrangian problem provides the gradient of $\Phi_\rho$, i.e. 
% \begin{equation}
%     \nabla \Phi_\rho(\Lambda) = - \sqrt{W_{neg}} X(\Lambda), \quad \text{where} \quad  X(\Lambda) = \argmin \left \{ F(X) + \sqrt{W_{neg}} \Lambda^T X +  \frac{\rho}{2}  \| X\|_{W_{neg}}^2 ) \right \} 
% \end{equation}
% Hence solving the subproblem inexactly directly translate to an inexact gradient of $\Phi_\rho$. Therefore, our proposed algorithm can be interpreted as applying inexact accelerated gradient method on the Moreau-envelope of the dual function. In other words, applying accelerated proximal point algorithm on the dual problem (\ref{dual}). Even though $F^*$ is strongly convex, $F^*(-\sqrt{W_{neg}} \Lambda)$ is not strongly convex with respect to $\Lambda$. It is only strongly convex restricted to the image space of $\sqrt{W_{neg}}$. To show the linear convergence rate, we need to show the update always lies in this subspace. 



% Therefore, by taking the approximation error as 
% \[ \epsilon_k = \frac{\mu \mu_\rho}{4} \sqrt{\frac{\mu_\rho}{L_\rho}} \Delta_0 \left (1- \frac{1}{2}\sqrt{\frac{\mu_\rho}{L_\rho}} \right )^k\]
% then 
% \[\Phi_{\rho}(\Lambda_k) - \Phi_{\rho}^*  \le C \left (1- \sqrt{\frac{\mu_\rho}{L_\rho}} \right )^k \Delta_0\]



==> [Neurips20] Decentralized Acc-AL algorithm /sections/sec5_exp.tex <==
\section{Experiments}
\setlength\belowcaptionskip{-2ex}
\begin{figure}[t]
\begin{subfigure}{.33\textwidth}
  \centering
    \includegraphics[width=\linewidth]{CircularGraphtau=1e-01}
%   \caption{\small Noise level}
%   \label{fig-main_correlation_cifar_lr01}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
    \includegraphics[width=\linewidth]{CircularGraphtau=1e+00}
%   \caption{\small Performance}
%   \label{fig-main_correlation_cifar_lr5}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
    \includegraphics[width=\linewidth]{CircularGraphtau=1e+01}
%   \caption{\small Performance}
%   \label{fig-main_correlation_cifar_lr5}
\end{subfigure}%
\\
\begin{subfigure}{.33\textwidth}
  \centering
    \includegraphics[width=\linewidth]{BarbellGraphtau=1e-01}
%   \caption{\small Noise level}
%   \label{fig-main_correlation_cifar_lr01}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
    \includegraphics[width=\linewidth]{BarbellGraphtau=1e+00}
%   \caption{\small Noise level}
%   \label{fig-main_correlation_cifar_lr01}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
    \includegraphics[width=\linewidth]{BarbellGraphtau=1e+01}
%   \caption{\small Performance}
%   \label{fig-main_correlation_cifar_lr5}
\end{subfigure}%
\caption{We evaluate the empirical performance of existing state-of-the-art algorithms, where the underlying network is a circular graph (top) and a barbell graph (bottom). We consider the following regimes: low communication cost (left), Ill-condition problems (middle) and High communication cost (right). The x-axis is the  time counter, i.e. the sum of the communication cost and the computation cost; the y-axis is the log scale suboptimality. We observe that our algorithms \our/M\our~are optimal under  
various regimes, validating our theoretical findings.}\label{fig:exps}
\end{figure}
\newcommand{\expnumber}[2]{{#1}\mathrm{e}{#2}}

Having described the \our/M\our{ }algorithms for  decentralized optimization problem \eqref{eq:global}, we now turn to presenting various empirical results which corroborate our theoretical analysis. To facilitate a simple comparison between existing state-of-the-art algorithms, we consider an $\ell_2$-regularized logistic regression task over two classes of the MNIST~\cite{lecun2010mnist} benchmark dataset.  The smoohtness parameter (assuming normalized feature vectors) can be shown to be bounded by $1/4$, which together with a regularization parameter $\mu\approx \expnumber{1}{-3}$, yields a relatively high $\expnumber{1}{3}$-bound on the condition number of the loss function. Further empirical results which demonstrate the robustness of ~\our/M\our\ under wide range of parameter choices are provided in Appendix~G.

We compare the performance of \our/M\our~with the state-of-the-art algorithms EXTRA \cite{shi2015extra}, APM-C \cite{li2018sharp} and the inexact dual method SSDA/MSDA \cite{scaman2017optimal}. We set the inner iteration counter to be $T_k=100$ for all  algorithms, %involving inner solver 
and use the theoretical stepsize schedule. The decentralized environment is modelled in a synthetic setting, where the communication time is steady and no latency is encountered. To  demonstrate the effect of the underlying  network architecture, we consider: a) a circular graph, where the agents form a cycle; b) a Barbell graph, where the agents are split into two complete subgraphs, connected by a single bridge (shown in Figure~2 in the appendix). %\ref{fig: Network-Samples}

% We do not address the practical implementation details nor the efficiency of the compared algorithms on real-world distributed platforms. The effect of latency, machine failures or variable communication time is thus left for future work.

% In this section, we conduct experiments to compare the performance of \our~with the state-of-the-art decentralized algorithms on two different network architectures: circular graph \bccomment{we said circular graph at legend} \hz{changed, Thanks for pointing this out} and Barbell graph. They have very different graph condition number $\kappa_{cycle} = O(n^2)$ but $\kappa_{barbell} = O(n)$\hz{Is the barbell graph condition number correct?} \mg{MG: It depends on how we take $W$. Do we choose $W=I-\alpha L$ where $L$ is the Laplacian?}. \hz{$W$ is the Laplacian, I changed the notation in the meanwhile since there is some subtlety in multi-stage} We focus on $\ell_2$-regularized logistic regression, where the regularization parameter $\mu$ yields a lower bound on the strong convexity parameter of the problem. We sample two classes of MNIST dataset and perform logistic regression on the normalized data. 


% We compare with EXTRA \cite{shi2015extra}, dual method SSDA+AGD \cite{scaman2017optimal} with gradient inexactly solved by AGD and its multistage variant MSDA+AGD \cite{scaman2017optimal} and  APM-C \cite{li2018sharp} near optimal primal algorithm, all the methods are implemented according to the theoretical choice of parameters. Fix the same number of inner loop for all inner-outer loop algorithm (only EXTRA is not) Observation: our method outperforms, dual method slow down due to the complexity of the inexact approximation

As shown in Figure \ref{fig:exps}, our multi-stage algorithm MIDEAL is optimal in the regime where the communication cost $\tau$ is small, and the single-stage variant \our~is optimal when $\tau$ is large. As expected, the inexactness mechanism  significantly slows down the dual method SSDA/MSDA in the low communication cost regime. In contrast, the APM-C algorithm performs reasonably well in the low communication regime, but performs relatively poorly when the communication cost is high. 










==> [Neurips20] Decentralized Acc-AL algorithm /sections/sec6_conclusion.tex <==
% \vspace{-0.2cm}
\section{Conclusions}
% \vspace{-0.2cm}
We propose a novel framework of decentralized algorithms for smooth and strongly convex objectives. The framework provides a unified viewpoint of several well-known decentralized algorithms and, when instantiated with AGD, 
achieves optimal convergence rates in theory and state-of-the-art performance in practice. We leave further generalization to (non-strongly) convex  and non-smooth objectives to future work.
%achieves  optimal convergence rates under wide range of parameter range, both theoretically and empirically. 

% \hz{no space}
% Mention some future direction like extension to convex but non-strongly convex setting, need a careful analysis, leave it as future work. 
